Estimation and Analysis of Slice Propagation Uncertainty in 3D Anatomy Segmentation

Supervised methods for 3D anatomy segmentation demonstrate superior performance but are often limited by the availability of annotated data. This limitation has led to a growing interest in self-supervised approaches in tandem with the abundance of available un-annotated data. Slice propagation has emerged as an self-supervised approach that leverages slice registration as a self-supervised task to achieve full anatomy segmentation with minimal supervision. This approach significantly reduces the need for domain expertise, time, and the cost associated with building fully annotated datasets required for training segmentation networks. However, this shift toward reduced supervision via deterministic networks raises concerns about the trustworthiness and reliability of predictions, especially when compared with more accurate supervised approaches. To address this concern, we propose the integration of calibrated uncertainty quantification (UQ) into slice propagation methods, providing insights into the model's predictive reliability and confidence levels. Incorporating uncertainty measures enhances user confidence in self-supervised approaches, thereby improving their practical applicability. We conducted experiments on three datasets for 3D abdominal segmentation using five UQ methods. The results illustrate that incorporating UQ improves not only model trustworthiness, but also segmentation accuracy. Furthermore, our analysis reveals various failure modes of slice propagation methods that might not be immediately apparent to end-users. This study opens up new research avenues to improve the accuracy and trustworthiness of slice propagation methods.

==> Old-method.tex <==
%\section{Estimating Uncertainty in Slice Propagation Techniques}
\section{Uncertainty in Slice Propagation}

% This section outlines various slice propagation techniques and our adaptations to incorporate different uncertainty quantification (UQ) methods discussed previously.

In this section, we provide a detailed overview of the two slice propagation methods, \textit{Sli2Vol} \cite{yeung2021sli2vol} and \textit{Vol2Flow} \cite{bitarafan2022vol2flow}, and describe how we integrated the different epistemic UQ methods into these frameworks.

\subsection{Slice Propagation Methods}

%We use two slice propagation methods namely (1) \textit{Sli2Vol}\cite{yeung2021sli2vol} and (2) \textit{Vol2Flow}\cite{bitarafan2022vol2flow}. 
% Both Sli2vol and Vol2Flow provide novel approaches for segmentation of 3D volumes using a single slice annotation. 
Sli2Vol \cite{yeung2021sli2vol} and Vol2Flow \cite{bitarafan2022vol2flow} are state-of-the-art approaches for segmentation of 3D volumes using a single slice annotation. 
% Let's assume two adjacent slices starting at z-direction $i$ are represented by $\mathbf{S}_i$ and $\mathbf{S}_{i+1}$. 
% Both the models outputs a deformation/correspondence matrix between the selected slices $\mathbf{A}_{i+1, i}$, which is then used to transform slice $i$, to get an estimate of slice $(i+1)$, difference between estimated and original slice is used for training the model. 
Both models operate by predicting a deformation/correspondence matrix between two adjacent slices, which is then used to propagate the segmentation. For example, given two adjacent slices at $z$-index $i$ and $i+1$, denoted $\mathbf{S}_i$ and $\mathbf{S}_{i+1}$, the models predict deformation matrix $\mathbf{A}_{i+1, i}$ which registers $\mathbf{S}_i$ to  $\mathbf{S}_{i+1}$. This matrix is then used to transform $\mathbf{S}_i$ to acquire an estimate of slice $(i+1)$, denoted $\hat{\mathbf{S}}_{i+1}$. The difference between the estimated slice, $\hat{\mathbf{S}}_{i+1}$, and the original slice, $\mathbf{S}_{i+1}$, is then used for model training. 
Sli2Vol doesn't give raw inputs to the network, rather they give multi-channel edges obtained via a edge profiling function denoted by $\mathcal{F}_E$.

\textbf{Sli2Vol.}\cite{yeung2021sli2vol} %Organ of Interest in a 3D volume, $V \in \mathbb{R}^{H \times W \times D}$, based on a 2D segmentation mask provided for a single slice, $M_i \in \mathbb{R}^{H \times W \times 1}$. 
Sli2Vol leverages learning feature representations to establish pixel-wise correspondences between adjacent slices, facilitating the propagation of the 2D slice mask across the volume through a set of learned affinity matrices, $\textbf{A}_{i \rightarrow i+1}$, in a self-supervised learning scheme.
Sli2Vol, used edges features and learn to register adjacent slices($\mathbf{S}_{i+1}$, $\mathbf{S}_i$) by producing Affinity/Warping matrices $\textbf{A}_{i \rightarrow i+1}$. The model is trained using an unsupervised MSE loss between the original Slice and reconstructed slice after warping.
%via  in an unsupervised manner via a convolution backbone.
%Sli2Vol involves training a ConvNet to reconstruct a slice from its neighbor using an edge profile generator, which forces the model to focus on edge information, thus avoiding trivial solutions and enhancing feature correspondence learning. During inference, the affinity matrices generated by the trained model are used to iteratively propagate the initial mask throughout the volume. Additionally, a verification module is proposed to correct the propagated masks at each step, minimizing error accumulation and improving segmentation accuracy.

\textbf{Vol2Flow}\cite{bitarafan2022vol2flow} introduces a self-supervised learning algorithm,  designed to segment 3D volumes based on a single slice annotation provided by the user. The algorithm leverages a large dataset of unlabeled volumes, treating each volume as a sequence of 2D slices to learn from the continuously evolving visual domain inherent in the data. Unlike traditional methods that rely on 2D CNN models for slice-by-slice transformation, Vol2Flow employs a 3D registration network to understand and apply a sequence of transformations across the entire volume, enabling dense segmentation mask generation for each test volume. Vol2Flow's architecture is inspired by 3D-UNet structures, producing two sets of Displacement Deformation Fields (DDFs) $\Phi^f = (\phi^f_{1,2}, \phi^f_{2,3}, \ldots, \phi^f_{D-1,D})$ and $\Phi^b = (\phi^b_{1,2}, \phi^b_{2,3}, \ldots, \phi^b_{D-1,D})$ for forward  and backward propagation of information between adjacent slices. The learning process involves generating neighboring slices around each source slice using the DDFs and minimizing a loss function that combines structural similarity index (SSIM) and an edge-preserving loss. $L(\tilde{x}_d, x_d) = \lambda (1 - \text{SSIM}(\tilde{x}_d, x_d)) + (1 - \lambda) \frac{1}{HW} \sum_{i=1}^{H} \sum_{j=1}^{W} C(x_d)_{i,j} |\tilde{x}_{d,i,j} - x_{d,i,j}|
$ This combination ensures the preservation of anatomical boundaries critical for segmentation. For mask propagation, Vol2Flow applies sequential transformations to generate pseudo labels for slices, introducing a refinement function to correct errors and enhance segmentation accuracy. The method  employs a non-linear classifier, specifically an SVM with an RBF kernel, to improve the classification of pixels during mask propagation, addressing the limitations of linear classification and reducing false positives.

%During training, \textit{Sli2Vol}\cite{yeung2021sli2vol} sets up a surrogate task of 2D registration of adjacent slices ($\mathbf{S}_i,\mathbf{S}_{i+1}$) to learn pixel-wise correspondences. The input to the correpondence flow  network are multi-channel edges of the two slices (computed using an edge profiling function $\mathcal{F}_E$), i.e., fixed ($\mathcal{F}_E(\mathbf{S}_{i+1}$)) and moving ($\mathcal{F}_E(\mathbf{S}_i)$). The output is the deformation/correspondence matrix ($\mathbf{A}_{i+1, i}$) beteewn the features from slices $(i+1,i)$. Deformation matrics is then used to register the two adjacent slices. The model is trained with the an MSE loss defined by:
%\begin{equation}
%    \mathcal{L} = ||\mathbf{S}_{i+1} - \mathbf{A}_{i+1,i}(\mathbf{S}_i) ||_2
%\end{equation}
%The loss above does not require any annotations and can be trained on a large amount of unannotated volumes. During inference, a single annotated slice(largest slice), which is annotated manually is given to the model, and using predicted correspondences $A_{i+1, i}$, the segmentation is propagated to the entire volume. Post-processing methods are used to control the error accumulation in segmented anatomy.

%\textit{Vol2Flow}\cite{bitarafan2022vol2flow}, is an extension of the above idea and is mainly different in three main aspects. First, instead of using multi-channel edges, \textit{Vol2Flow} use raw pixel values. Second, for obtaining the correspondence matrices ($A_{i+1, i}$), \textit{Vol2Flow} does not use a single adjacent slice but rather the entire volume (N slices) to create dense correspondence matrices for both directions of the volume ($\pm$ z-direction). Third, the model is trained using a structural similarity index (SSIM) and an edge-preserving loss. The inference module is similar, except the post-processing module is modified to a pixel classifier model on the manually annotated slice. %For more details, we refer the reader to the original text. 

%\subsection{Methods for Quantifying Epistemic Uncertainty}
\subsection{Epistemic Uncertainty Quantification}

% \ja{JADIE:- Please review this whole section. Make the modification necessary. We have used a decent amount of language from your paper. Maybe you can modify the content so that it is slightly different.}
%While the scalable estimation of epistemic uncertainty has been explored in supervised segmentation models \cite{adams2023benchmarking}, its application in slice propagation techniques remains under-explored. To bridge this gap, we investigate five distinct UQ methods, each described below. 
%Quantifying epistemic uncertainty in deep learning models presents significant challenges, particularly due to the complexity and variability inherent in high-dimensional data spaces \cite{}. 
While considerable progress has been made in estimating epistemic uncertainty within supervised segmentation models \cite{adams2023benchmarking}, extending these advancements to slice propagation techniques has not been studied. We adapt and evaluate the effectiveness of different epistemic UQ methods specifically for slice propagation tasks. These UQ methods for uncertainty quantification are crucial for the reliable application of slice propagation techniques in clinical applications. In this section, we provide detailed steps for adapting the choosen UQ methods for slice propagation. 
%By focusing on this under-explored area, we aim to provide insights that can help bridge the gap between theoretical UQ models and practical, real-world applications in medical imaging.

%\textbf{Deep Ensemble} \cite{lakshminarayanan2017simple} involves training multiple independent networks with random initialization and averaging their predictions in inference. This approach was proposed to improve prediction accuracy and robustness and serves as a frequentist approach for epistemic UQ. The spread in predictions made by various ensemble members captures model uncertainty. Deep ensembles require training and storing multiple models, inhibiting scalability and limiting the applicability of this method to large networks.

The \textbf{Deep Ensemble} method \cite{lakshminarayanan2017simple} enhances prediction accuracy and robustness by leveraging the diversity in predictions from multiple independently trained Slice propagation models.
%This approach, which aggregates predictions from networks initialized randomly, serves as a practical frequentist method for quantifying epistemic uncertainty. 
This method serves as an effective frequentist approach for quantifying epistemic uncertainty by aggregating predictions across multiple models. Specifically, aggregation is achieved by averaging the outputs of the ensemble members. The variability in the ensemble's predictions reflects the model's uncertainty. We used four different initialization to train models (1) base initialization, similar to original implementations; (2) Kaiming (He) uniform initialization (3) Glorot (Xavier) uniform initialization and (4) custom normal initialization.  These strategies ensure each model in the ensemble explores different data representations, enhancing the ensemble's generalization capabilities and providing a more nuanced measure of uncertainty

%Despite its effectiveness in improving performance and generalization—since different models capture various aspects of the data—the method's scalability is challenged by its high computational and memory demands, particularly for large networks.

%To mitigate these limitations, our implementation focuses on optimizing the initialization phase to foster model diversity without excessively burdening computational resources. We adopted four distinct initialization strategies for the ensemble's models, tailored to the Sli2Vol and Vol2Flow architectures: (1) Base Initialization, as in their released implementaions; (2) Kaiming (He) Uniform Initialization for convolutional layers, particularly beneficial for those followed by ReLU activations to prevent vanishing/exploding gradients; (3) Glorot (Xavier) Uniform Initialization for convolutional layers to maintain consistent gradient scales across layers; and (4) Custom Normal Initialization, applying a normal distribution with a specific standard deviation for convolutional layers and uniform initialization for batch normalization layers' weights. These strategies ensure each model in the ensemble explores different data representations, enhancing the ensemble's generalization capabilities and providing a more nuanced measure of uncertainty, thus balancing the deep ensemble method's resource demands with the practical constraints of computational and storage capacities.


%The \textbf{Deep Ensemble} method \cite{lakshminarayanan2017simple}, enhances prediction accuracy and robustness by leveraging the diversity in predictions from multiple independently trained networks. This approach, which aggregates predictions from networks initialized randomly, serves as a practical frequentist method for quantifying epistemic uncertainty. The variability in the ensemble's predictions reflects the model's uncertainty, offering insights into the confidence of its outputs. Despite its effectiveness in improving performance and generalization—since different models capture various aspects of the data—the method's scalability is challenged by its high computational and memory demands, particularly for large networks.

%To mitigate these limitations, our implementation focuses on optimizing the initialization phase to foster model diversity without excessively burdening computational resources. We adopted four distinct initialization strategies for the ensemble's models, tailored to the Sli2Vol and Vol2Flow architectures: (1) Base Initialization, as in their released implementaions; (2) Kaiming (He) Uniform Initialization for convolutional layers, particularly beneficial for those followed by ReLU activations to prevent vanishing/exploding gradients; (3) Glorot (Xavier) Uniform Initialization for convolutional layers to maintain consistent gradient scales across layers; and (4) Custom Normal Initialization, applying a normal distribution with a specific standard deviation for convolutional layers and uniform initialization for batch normalization layers' weights. These strategies ensure each model in the ensemble explores different data representations, enhancing the ensemble's generalization capabilities and providing a more nuanced measure of uncertainty, thus balancing the deep ensemble method's resource demands with the practical constraints of computational and storage capacities.

%\textbf{Batch Ensemble} \cite{wen2020batchensemble} was proposed as a method to leverage the advantages of ensemble learning without compromising scalability. Batch ensemble reduces the computational and memory cost by defining each weight matrix as a Hadamard product of a shared weight and member-specific vectors. Ensemble members are distinguished by lightweight rank-one vectors, rather than entire networks.  

The \textbf{Batch Ensemble} method \cite{wen2020batchensemble} improves on traditional deep ensemble approaches by significantly reducing the computational and memory demands. Assuming $N$ as number of ensemble methods.
%Each weight matrix forms the Hadamard product of shared base weights and model-specific rank-one vectors, allowing for parameter sharing across ensemble members. 
Batch ensemble represents each weight convolutional weight matrix in slice propagation models $\mathbf{W}$, of the ensemble as the Hadamard product ($\circ$) of a shared base weight matrix $\mathbf{W}_{\text{shared}}$ and two model-specific rank-one vectors, $\mathbf{r_i}$ and $\mathbf{s_i}$, where $i=1,2,..N$. The  mathematical formulation for the weight matrix of each ensemble member $i$ is given by $\mathbf{W}_i = \mathbf{r}_i \circ \mathbf{W}_{\text{shared}} \circ \mathbf{s}_i^T$. %where $\mathbf{r}_i$ and $\mathbf{s}_i$ are vectors specific to each ensemble member, representing the `fast' and `slow' weights, respectively.
%This setup enables simultaneous training of multiple models, each capturing unique data aspects through a blend of shared and individual weights, enhancing efficiency without significantly compromising performance or uncertainty estimation. We introduce ensemble-specific rank-one parameters (fast and slow weights) during the initialization of convolutional and batch normalization layers, enabling the model to support ensemble dynamics. %The forward pass is adjusted to utilize these parameters, ensuring each ensemble member's distinctiveness influences the model's output. 
%Our implementation includes a specialised convolutional layer that introduces these ensemble-specific parameters during initialization. By applying the ensemble-specific scaling $r_i$ and $s_i$ to the shared weights $W_{\text{shared}}$, we enable each model within the ensemble to learn unique data representations while sharing a common computational backbone, thus enhancing both efficiency and model performance without significantly impacting uncertainty estimation.
%Ensemble averaging is streamlined through batch operations, facilitating efficient computation of averaged predictions across members during inference, where the model generates predictions for four samples, demonstrating the method's balance between scalability and robust predictive performance.
%For ensemble averaging, we employ batch operations \cite{wen2020batchensemble} to efficiently compute the averaged predictions across all ensemble members during inference. This involves extending the input across the ensemble dimension, applying the model-specific transformations through the adjusted weight matrices, and then averaging these outputs to obtain the final prediction. 
We compute the averaged predictions across all ensemble members during inference. This involves extending the input across the ensemble dimension, applying the model-specific transformations through the adjusted weight matrices, and then averaging these outputs to obtain the final prediction. 

%The \textbf{Batch Ensemble} method \cite{wen2020batchensemble}, innovates ensemble learning by reducing its computational and memory footprint. It achieves this by constructing each weight matrix from the Hadamard product of shared base weights and model-specific rank-one vectors, allowing for parameter sharing across ensemble members. This setup enables simultaneous training of multiple models, each capturing unique data aspects through a blend of shared and individual weights, enhancing efficiency without significantly compromising performance or uncertainty estimation.

%Our implementation introduces ensemble-specific rank-one parameters (fast and slow weights) during the initialization of convolutional and batch normalization layers, enabling the model to support ensemble dynamics. The forward pass is adjusted to utilize these parameters, ensuring each ensemble member's distinctiveness influences the model's output. Ensemble averaging is streamlined through batch operations, facilitating efficient computation of averaged predictions across members during inference, where the model generates predictions for four samples, demonstrating the method's balance between scalability and robust predictive performance.

%\textit{Monte Carlo (MC) Dropout} sampling \cite{gal2016dropout} is the most common Bayesian technique for uncertainty quantification. Dropout is a fast scalable approach to approximate variational inference that has been shown to produce accurate uncertainty estimates in classification, regression, segmentation, and reinforcement learning tasks \cite{gal2016dropout,adams2023benchmarking,adams2020uncertain}.  This method entails applying dropout to every network layer and sampling multiple predictions with various dropout masks in inference to acquire a distribution. The variance of the predicted distribution captures model uncertainty.  

\textbf{Monte Carlo (MC) Dropout} \cite{gal2016dropout} is a widely used technique for measuring uncertainty in predictive models, inspired by Bayesian principles. MC Dropout involves randomly omitting parts of the model's information flow during each prediction phase, enabling the model to produce a range of possible outcomes for the same input. This variability offers a glimpse into the model's certainty levels. For slice propagation methods, we customized dropout layer placements within residual networks blocks, positioning them post-ReLU activation \cite{adams2020uncertain} to enrich uncertainty estimates. We optimized the dropout probability at 0.2 during training for a balance between randomness and learning efficiency. %Uniquely, we kept the model in training mode during inference, conducting 30 forward passes to generate a diverse set of predictions. This strategy allowed us to capture a broad spectrum of uncertainty, providing a more nuanced understanding of the model's confidence across high-dimensional data. These adaptations not only improved the precision of uncertainty quantification but also enhanced the method's applicability to complex slice propagation tasks, facilitating more informed decision-making in critical applications.

%\textbf{Monte Carlo (MC) Dropout} \cite{gal2016dropout} is a widely used technique for measuring uncertainty in predictive models, inspired by Bayesian principles. This method, recognized for its simplicity and effectiveness, approximates complex statistical processes to estimate how confident a model is about its predictions. It has proven its merit across various tasks, including classification, regression, and segmentation, by providing accurate uncertainty estimates \cite{gal2016dropout,adams2023benchmarking,adams2020uncertain}. At its core, MC Dropout involves randomly omitting parts of the model's information flow during each prediction phase, enabling the model to produce a range of possible outcomes for the same input. This variability offers a glimpse into the model's certainty levels.

%In enhancing the Monte Carlo (MC) Dropout method for slice propagation, we customized dropout layer placements within Residual Networks Blocks, positioning them post-ReLU activation to enrich uncertainty estimates. We optimized the dropout probability at 0.2 during training for a balance between randomness and learning efficiency. Uniquely, we kept the model in training mode during inference, conducting 30 forward passes to generate a diverse set of predictions. This strategy allowed us to capture a broad spectrum of uncertainty, providing a more nuanced understanding of the model's confidence across high-dimensional data. These adaptations not only improved the precision of uncertainty quantification but also enhanced the method's applicability to complex slice propagation tasks, facilitating more informed decision-making in critical applications.

%\textit{Concrete Dropout} \cite{gal2017concrete} is an extension of MC dropout, proposed to address the challenge of dropout rate tuning. Acquiring well-calibrated uncertainty estimates via MC dropout requires performing a costly grid search to tune layerwise dropout rates.  Concrete Dropout \cite{gal2017concrete} uses a continuous relaxation of dropout discrete masks to enable automatically optimizing dropout probabilities along with network weights. 

\textbf{Concrete Dropout} \cite{gal2017concrete}, addresses the challenge of manually tuning dropout rates in MC dropout which can be both time-consuming and computationally expensive. By employing a continuous relaxation of the dropout's discrete masks, concrete dropout allows for the automatic optimization of dropout probabilities in tandem with network weights, significantly streamlining the process. For slice propagation methods we integrated concrete dropout with all convolutional layers present in slice propagation networks ensuring dropout probabilities are optimally tuned without manual intervention. %Our implementation enriches the model's ability to provide nuanced uncertainty estimates, particularly in complex slice propagation tasks, by embedding Concrete Dropout directly into the model architecture, thus facilitating a more efficient and effective uncertainty quantification process.

%\textbf{Concrete Dropout} \cite{gal2017concrete}, an advanced iteration of MC Dropout, addresses the challenge of manually tuning dropout rates—a process that can be both time-consuming and computationally expensive. By employing a continuous relaxation of the dropout's discrete masks, Concrete Dropout innovatively allows for the automatic optimization of dropout probabilities in tandem with network weights, significantly streamlining the process. In our work, we leveraged this technique to automatically adjust dropout rates, specifically wrapping convolutional layers within Residual Network Blocks to enhance model reliability and uncertainty calibration. This was achieved by integrating Concrete Dropout with convolutional layers, followed by batch normalization and ReLU activation, ensuring dropout probabilities are optimally tuned without manual intervention. Our implementation enriches the model's ability to provide nuanced uncertainty estimates, particularly in complex slice propagation tasks, by embedding Concrete Dropout directly into the model architecture, thus facilitating a more efficient and effective uncertainty quantification process.

%An alternative approach for mitigating the computational complexity of deep ensemble methods is stochastic weight averaging (SWA) \cite{izmailov2018averaging}. SWA defines the final model weights as the average of weights traversed during stochastic gradient descent (SGD) after initial convergence. SWA enables acquiring a distribution of model weights and associated predictions by simply training a the model for an extended duration and retaining the weights.
%\textit{SWA Gaussian} (SWAG) \cite{maddox2019simple}, extended this approach for UQ by fitting a Gaussian distribution on the sampled weights. This serves as a posterior distribution over weights that provides an output distribution.

\textbf{Stochastic Weight Averaging Gaussian (SWAG)} \cite{maddox2019simple} builds upon SWA \cite{izmailov2018averaging} by averaging model weights over the latter part of training to find a broader optimum and fitting a Gaussian distribution over these averaged weights to model the posterior distribution of the weights. The posterior estimation facilitates the generation of diverse predictions that reflect the uncertainty in the model's outputs. We obtained the mean weights and their post-convergence covariance matrices during training to estimate the underlying gaussian weight distribution for slice propagation. We sampled these distribution during to obtain different weight parameters, enabling the generation of varied predictions needed uncertainity estimation.

%In our study, we adopted and extended the \textbf{Stochastic Weight Averaging Gaussian (SWAG)}\cite{maddox2019simple} approach to enhance uncertainty quantification (UQ) in deep learning models. SWAG builds upon \textbf{Stochastic Weight Averaging (SWA)}\cite{izmailov2018averaging} by not only averaging model weights over the latter part of training to find a broader optimum but also by fitting a Gaussian distribution over these averaged weights to model the posterior distribution of the weights. This method allows for a more nuanced capture of the model's weight distribution, facilitating the generation of diverse predictions that reflect the uncertainty in the model's outputs.

%To implement this, we integrated SWA into our training regimen to average weights after a predefined epoch, enhancing the model's generalization by exploring wider optima in the loss landscape. Beyond SWA, we extended our approach to include SWAG by estimating the covariance matrix of the weights post-convergence. This was achieved by collecting weight samples and calculating the outer product of deviations from the SWA mean, thus approximating the posterior weight distribution.

%For inference, we leveraged the mean weights and covariance matrix obtained via SWAG to sample new sets of model parameters, enabling the generation of varied predictions. This approach not only provided a practical method for UQ but also improved the robustness and reliability of our model by capturing and utilizing the inherent weight distribution variance during training.

% \ja{JADIE: I couldn't think of a better way to say why we didn't include other methods. do you think this is fine ??}Other UQ methods were not included in the analysis because their performance was similar to the methods included in the study. Including those methods in the analysis doesn't affect the conclusions drawn from this work.  
%Additional methods of UQ have been proposed, such as Bayesian neural nets  \cite{dusenberry2020rank1,franchi2020encoding}, as well as approximate inference approaches such as Bayes by Backprop \cite{blundell2015weight} and sampling-based Markov chain Monte Carlo \cite{chen2014stochastic}. Such approaches are excluded from this benchmark as they have limited scalability, tend to underfit, and previous work has shown they are comparable to more lightweight techniques \cite{adams2023benchmarking,dusenberry2020rank1,gal2016dropout,lakshminarayanan2017simple}.

%While additional UQ methods, such as Bayesian neural networks \cite{dusenberry2020rank1,franchi2020encoding} and approximate inference techniques like Bayes by Backprop \cite{blundell2015weight} and Markov chain Monte Carlo (MCMC) \cite{chen2014stochastic}, have been proposed, they were not included in our benchmark analysis. This decision was based on comprehensive preliminary assessments indicating that these methods offer performance comparable to the ones we selected, without significantly altering the study's conclusions. Furthermore, issues such as limited scalability, a tendency to underperform in certain contexts, and equivalence in effectiveness to more computationally efficient techniques \cite{adams2023benchmarking,dusenberry2020rank1,gal2016dropout,lakshminarayanan2017simple} informed our selection process. Our focus was on methods that balance scalability, computational efficiency, and robustness in uncertainty estimation, ensuring the relevance and applicability of our findings to a broad range of practical scenarios.


\subsection{Evaluation Metrics}

% \rn{Self Note: Add other metrics if decided to report}

%We report dice similarity score, a frequently employed metric to gauge the performance of segmentation networks \cite{kataria2023automating,kataria2023pretrain,ronneberger2015u,chen2017rethinking}. 
%We also report Variation of Information to assess the consistency and accuracy of the propagation process by quantifying the change in information content between the original and propagated segmentations.

%We evaluate the Pearson correlation coefficient ($r$) between epistemic uncertainty and prediction error (100-dice), which measures uncertainty calibration. A higher correlation value indicates the model is better calibrated. We also use error-retention curves to jointly access segmentation accuracy and uncertainty quantification. We report the area under the error retention curve(R-AUC) using (100-dice) as the error metric as done by other uncertainty methods \cite{adams2023benchmarking}. 

We utilize the \textbf{Dice Similarity Coefficient (DSC)}, a widely recognized metric for evaluating segmentation network performance \cite{kataria2023automating,kataria2023pretrain,ronneberger2015u,chen2017rethinking}.
%that measures the voxel-wise overlap between a predicted segmentation and its groundtruth as follows:
%$$DSC = \frac{2 \times |X \cap Y|}{|X| + |Y|}$$
%where $X$ and $Y$ represent the set of voxels in the ground truth and predicted segmentation resepectively.
To understand how well the predicted segmentation conforms to the actual boundaries as defined by the ground truth, we report the \textbf{Average Surface Distance (ASD)} which is calculated as:
$$\text{Average Distance}_{\text{groundtruth to prediction}} = \frac{\sum_{i} (d_i \times a_i)}{\sum_{i} a_i}$$
where $d_i$ is the distance of the $i$-th surface element from the ground truth to the nearest point on the predicted surface, and $a_i$ is the area (or length in 2D) of the $i$-th surface element on the ground truth.

%The ASD is calculated by first computing the distance from each surface element of the groundtruth to the nearest surface element in the predicted mask, then weighing them by the surface element areas to compute an average that reflects the geometric properties of the surfaces. 
%Variation of Information to measure the consistency and precision of segmentation propagation by quantifying informational changes between original and propagated segmentations.

Furthermore, we assess model calibration through the \textbf{Pearson correlation coefficient ($r$)} between epistemic uncertainty and prediction error (100-dice), where a higher $r$ value signifies better calibration, defined as:
$$r = \frac{\sum (x_i - \bar{x})(y_i - \bar{y})}{\sqrt{\sum (x_i - \bar{x})^2 \sum (y_i - \bar{y})^2}} $$
where $x_i$ represents the epistemic uncertainty and $y_i$ represents the prediction error (100 - DSC) for the $i$-th prediction with means $\bar{x}$ and $\bar{y}$.

%To jointly evaluate segmentation accuracy and uncertainty quantification, we employ error-retention curves, reporting the area under the curve (R-AUC) with (100-dice) as the error metric, aligning with practices in existing uncertainty quantification research \cite{adams2023benchmarking}.

Error-retention curves plot the prediction error (100 - DSC) against the proportion of data retained after excluding predictions with the highest uncertainty. To jointly evaluate segmentation accuracy and uncertainty quantification, we report the area under this curve \textbf{(R-AUC)} which quantifies the model's performance across different levels of uncertainty retention. A lower R-AUC indicates better performance, as it implies lower error across retained predictions.


